AGN's Deadness Over Cosmic Time: UVJ Diagrams of X-Ray-Selected AGN

Active Galactic Nuclei (AGN) are intensely accreting supermassive black holes at the centers of massive galaxies. Though these objects occupy little spatial extent of the galaxy itself, they are thought to have far reaching affects, impacting the galaxy's star formation, and possibly it's lifespan until it becomes 'red and dead'. Typical galaxies demonstrate that, over cosmic time, they tend to separate into a bimodal distribution of 'red and dead' or blue and star forming. We examine whether active galaxies evolve over cosmic time in a similar way, and whether this can reveal anything about the complexities of the relationship between an AGN and the host galaxy. We use the Stripe82X survey to identify 3940 X-ray AGN spanning z=0-2.5, and we measure the rest-frame UVJ colors of each galaxy. We classify AGN as star-forming or quiescent based on their location in a UVJ color diagram. We find that there is not a clear bimodal distribution between AGN in star forming and quiescent galaxies. Furthermore, the most luminous X-ray sources tend to lie in the star forming region, which may indicate a correlation between central engine activity and increased rates of star formation.

==> name.tex <==
last intro sentence 

This paper aims to investigate the first question by assessing  the ratio of quiescent to star-forming active galaxies over cosmic time, in a manner similar to the assessment done of non-active galaxies in \cite{Williams}.

Here, the same binned diagrams will be generated from a survey of X-Ray selected AGN from the Stripe 82X survey (\cite{Ananna_2017}).  

\\ \indent One of the principle aspects of host galaxies that can be affected by their AGN is star formation rate. To investigate the star formation rate of the galaxies hosting our x-ray selected AGN, we use UVJ diagrams. These are utilized in \cite{Williams}, where star formation of non-active galaxies is assesed based on their placement on a color-color diagram. One axis corresponds to the brightness of the source in the U band subtracted by the brightness in the V band, and the other axis is the same, but with the V and J bands. This type of diagram has an empirically based limit between which one can determine whether a galaxy is star forming or quiescent. The authors demonstrated that over cosmic time, galaxies have become more bimodal in their quiescent (‘red’) and star forming (‘blue) distributions \cite{Williams}. 

To achieve this using the given survey data, the photometric data from each source must be fit to an empirical spectral energy distribution (SED) to be able to find the probable brightness of each source in the relevant rest-frame colors for our analysis (U, V and J band brightness). To cross check the validity of the results, two sets of plots will be made- one with the sources fit using only their optical data, and the SEDs given from the survey data, with a program written by the author. Second, the sources and their entire wavelength information will be fit to a much larger array of SEDs and parameters through the program XCigale (\cite{Yang_2022}), specifically intended for fitting photometric data that has prominent X-ray emission. The two will be compared to ensure that any conclusions drawn from this analysis can be made in good faith.
